ICON$^2$: Reliably Benchmarking Predictive Inequity in Object Detection

As computer vision systems are being increasingly deployed at scale in high-stakes applications like autonomous driving, concerns about social bias in these systems are rising. Analysis of fairness in real-world vision systems, such as object detection in driving scenes, has been limited to observing predictive inequity across attributes such as pedestrian skin tone, and lacks a consistent methodology to disentangle the role of confounding variables e.g. does my model perform worse for a certain skin tone, or are such scenes in my dataset more challenging due to occlusion and crowds? In this work, we introduce ICON$^2$, a framework for robustly answering this question. ICON$^2$ leverages prior knowledge on the deficiencies of object detection systems to identify performance discrepancies across sub-populations, compute correlations between these potential confounders and a given sensitive attribute, and control for the most likely confounders to obtain a more reliable estimate of model bias. Using our approach, we conduct an in-depth study on the performance of object detection with respect to income from the BDD100K driving dataset, revealing useful insights.

==> sections/table_exp_attr.tex <==
\begin{table*}[b!]
\centering
%%%     Car Ranking     %%%
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{r| cc cc cc cc cc }
    \toprule
    &  \multicolumn{2}{c}{Traffic Sign}& \multicolumn{2}{c}{Traffic Light}& \multicolumn{2}{c}{Bus}& \multicolumn{2}{c}{Motorcycle} & \multicolumn{2}{c}{Bicycle}\\
    \cmidrule(l{4pt}r{4pt}){2-3}
    \cmidrule(l{4pt}r{4pt}){4-5}
    \cmidrule(l{4pt}r{4pt}){6-7}
    \cmidrule(l{4pt}r{4pt}){8-9}
    \cmidrule(l{4pt}r{4pt}){10-11}
    \cmidrule(l{4pt}r{4pt}){12-13}
    \small{Rank}   & \small{$E$} & \small{$\sigma(\text{ProxyAP}^\Da)$} & \small{$E$} & \small{$\sigma(\text{ProxyAP}^\Da)$}  & \small{$E$} &\small{$\sigma(\text{ProxyAP}^\Da)$}  & \small{$E$} &\small{$\sigma(\text{ProxyAP}^\Da)$}  & \small{$E$} &\small{$\sigma(\text{ProxyAP}^\Da)$}  \\
    \midrule
    \texttt{1}     & size     & 0.214  & time      & 0.230  & size      & 0.881  & size      & 0.372  & size      & 0.715 \\
    \texttt{2}     & weather  & 0.159  & size      & 0.205  & occlusion & 0.700  & occlusion & 0.293  & weather   & 0.456 \\
    \texttt{3}     & occlusion& 0.119  & scene     & 0.061  & weather   & 0.242  & weather   & 0.138  & time      & 0.388 \\
    \texttt{4}     & time     & 0.069  & weather   & 0.060  & scene     & 0.239  & scene     & 0.032  & occlusion & 0.201 \\
    \texttt{5}     & scene    & 0.021  & occlusion & 0.068  & time      & 0.060  & time      & 0.023  & scene     & 0.041 \\
    \bottomrule
\end{tabular}
}
\caption{Explanatory attribute output ranking for the remaining 5 classes in the BDD-100K dataset. Note: all proxyAP variance values are smaller than the discovered explanatory attributes for car, pedestrian, truck (Table~\ref{table:control_results}) and hence we did not find a compelling explanation for our sensitive attribute (income), however for the bus, motorcycle, bicycle classes the counts are too low to compute reliable AP values. }
\label{table:darankings}
\end{table*}

